Vision-Language Pre-training: Basics, Recent Advances, and Future Trends

This paper surveys vision-language pre-training (VLP) methods for multimodal intelligence that have been developed in the last few years. We group these approaches into three categories: ($i$) VLP for image-text tasks, such as image captioning, image-text retrieval, visual question answering, and visual grounding; ($ii$) VLP for core computer vision tasks, such as (open-set) image classification, object detection, and segmentation; and ($iii$) VLP for video-text tasks, such as video captioning, video-text retrieval, and video question answering. For each category, we present a comprehensive review of state-of-the-art methods, and discuss the progress that has been made and challenges still being faced, using specific systems and models as case studies. In addition, for each category, we discuss advanced topics being actively explored in the research community, such as big foundation models, unified modeling, in-context few-shot learning, knowledge, robustness, and computer vision in the wild, to name a few.

==> 2_basics.tex <==
\chapter{Tasks, Benchmarks, and Early Models}
\label{chp:basics}

% [Jianfeng: we might add a section to introduce CV tasks, and how they can be cast as VL tasks, as we described in Chapter 1 -- Vision tasks as VL problems? Also consider whether we need a separate chapter on VL tasks/benchmarks or we can describe the tasks/datasets in the following chapters. We might merge this chapter with chapter 3 to provide the background of VL modeling (encoding images, texts, fusing image and text, answer generation.) ]

In this chapter, Section~\ref{chp2-sec:task-datasets} introduces major vision language (VL) tasks and the benchmarks that are commonly used in the research community. We group these tasks into two categories. VL understanding tasks, such as image-text retrieval and vision question answering (VQA), require a VL model to \emph{select} the output from a given list of candidates. VL generation tasks, such as image captioning and text-to-image generation, require a VL model to \emph{generate} the output.  

In Section~\ref{chp2-sec:evaluation}, we describe how to measure the quality of machine learning models on various VL tasks. While models for understanding tasks can be easily evaluated by comparing the model-selected output with the gold output, evaluation on generation tasks is challenging since the gold output is often not unique, \textit{e.g.,} in image captioning, there are often multiple plausible captions for an input image.   

In Section~\ref{chp2-sec:basics}, we describe language and vision processing techniques that serve as the building blocks of the VLP methods described in the later chapters, including text feature extraction, vision feature extraction, and language and vision feature fusion.

In Section~\ref{chp2-sec:task-specific-models}, we use VQA and image captioning as examples to review task-specific VL models that had been developed before large-scale pretrained language models and VLP methods are widely used for VL tasks. These early VL models are still used not only as baselines to demonstrate the (dis)advantages of the VLP methods being developed, but also to provide task-specific insights to help design pre-trained VL models that can be adapted efficiently to downstream tasks.   

%\section{Image-Text Understanding Tasks}
% vqa, gqa, nlvr2, ve, all the robustness benchmarks (refer to section 3, advanced topics?), vcr, and other reasoning tasks.

%\section{Image-Text Generation Tasks}
%captioning, paragraph captioning, visual storytelling etc. 

%\section{Video-Text Understanding and Generation Tasks}

\section{Tasks and Datasets}
\label{chp2-sec:task-datasets}
Casting as machine learning tasks, VL tasks can be formulated as $y = f(x;\theta)$, where we aim to learn a VL model $f$, parameterized by $\theta$, to generate output $y$ for input $x$. VL tasks can be categorized along two dimensions. 
Depending on the modalities of $x$ and $y$, VL tasks can be grouped into image-text or video-text tasks. 

Depending on how $y$ is generated by $f$, VL tasks can be grouped into \emph{understanding} task, such as image-text matching and vision question answering (VQA), where $y$ is selected by $f$ from a given candidate list, and \emph{generation} tasks, such as image captioning, where $y$ needs to be generated by $f$.

\begin{figure*}[t!]
  \centering
    \includegraphics[width=0.6\linewidth]{figs/chp2_vqa.jpg}
  \caption{Illustration of the VQA task. Figure credit: \citet{goyal2017making}.}
  \label{fig:chp2_vqa}
\end{figure*}

\begin{figure*}[t!]
  \centering
    \includegraphics[width=0.6\linewidth]{figs/chp2_image-captioning.jpg}
  \caption{Illustration of the image captioning task. Figure credit: \citet{chen2015microsoft}.}
  \label{fig:chp2_image-captioning}
\end{figure*}

We summarize all the VL tasks that are described in this paper in Table 1, where for each task we present its input modality, output modality, benchmark datasets, evaluation metrics, and the chapter where it is described. 
The VQA task is illustrated in Figure~\ref{fig:chp2_vqa}, where the model needs to answer the question regarding an image. VQA is considered as a understanding task because the answer is selected from a set of candidates that are given.
The image captioning task is illustrated in Figure~\ref{fig:chp2_image-captioning}, where the model needs to generate a free-form textual caption of an image. 
Note that we also include in Table 1 three tasks that are traditionally treated as computer vision tasks: image classification (IC), object detection (OD), and image segmentation (IS). 
%As described in Chapter 4, recent studies show that VL models trained on free-form language supervision data achieve very good results on these tasks, in particular in open-vocabulary settings.
IC or OD is traditionally defined as an understanding task since the image classes or object categories to be assigned to an input image are pre-defined, as on the ImageNet or COCO benchmarks. Recently, there is an growing interest in open-vocabulary IC and OD
\footnote{https://computer-vision-in-the-wild.github.io/eccv-2022/}, where image classes and object labels are not pre-defined but need to be generated on-the-fly given an input image, thus turning IC and OD to generation tasks, like image captioning. 
Image segmentation involves grouping image pixels and assigning a class category to each pixel. Similar to OD and IC, IS can be treated as an understanding or generation task depending on whether there is a pre-defined set of class categories.
As to be described in Chapter 4, although the three tasks are traditionally handled using vision models, recent studies show that VL models trained on free-form language supervision data achieve very good results on these tasks, particularly in open-vocabulary settings.

[Table 1:]

%and the corresponding datasets that are commonly used in the research community for model development and evaluation in Table 1. The summary covers the tasks described in recent survey papers \citep[e.g.,][]{li2022vision,chen2022vlp,du2022survey}, and all the tasks which will be described in the later chapters. 
\section{Evaluation Metrics}
\label{chp2-sec:evaluation}

Understanding tasks can be easily evaluated by comparing the model-selected output with the gold output using metrics such as precision, recall, and F-score.

Evaluation on generation tasks is challenging since the gold output is often not unique. For example, in image captioning, there are often multiple plausible captions for an input image. We present a brief review of the evaluation metrics used to measure the quality of model-generated texts and images. Recent reviewers include \citet{celikyilmaz2020evaluation,luo2021survey}.

\subsection{Evaluation of Text Generation}
Consider image captioning as illustrated in Figure~\ref{fig:chp2_image-captioning}. The task is to generate for a given image a textual caption that is not only \emph{fluent} as human-generated text but \emph{relevant} as to form a good description of the image content. Metrics used to evaluate the fluency and relevance can be grouped into three categories, according to \citet{celikyilmaz2020evaluation}.

\subsubsection*{Human Evaluation}
It is generally agreed in the research community that the most reliable way to evaluate the quality of model-generated text is to involve humans as judges. Naive or expert subjects are asked to rate model-generated text via 
\begin{itemize}
    \item \textbf{intrinsic evaluation:} how much the text looks like human-generated ones in terms of fluency, diversity, informativeness, etc., and
    \item \textbf{extrinsic evaluation:} how good the text serves the purpose of describing the image in terms of relevance, factuality, usefulness, etc.
\end{itemize}

However, human evaluation faces three challenges \citep{celikyilmaz2020evaluation}.
First, it is very expensive and time-consuming to run. Although the use of online crowd-sourcing platforms such as Amazon Mechanical Turk significantly improves the efficiency of human evaluation, quality control is difficult. 
Second, some dimensions of generated text quality that are not well-suited to human evaluation, such as diversity~\citep{hashimoto2019unifying}. 
Third, there is a lack of consistency or consensus among researchers working on the same topic how human evaluation is performed and how the result is presented. For example, \citet{van2021human} find that in a sample of natural language generation papers from ACL and INLG, only 57\% of papers report the number of participants in their human evaluations. This makes it difficult to reproduce experiments or compare results reported by others.

\subsubsection*{Automatic Metrics}

This is most commonly used in the research community. 
Unlike human evaluation, automatic evaluation is typically performed on pre-collected datasets (benchmarks) without human in the loop. Thus, it is inexpensive to run the evaluation repeatedly to monitor research progress. The result reported by one group can be easily re-produced for comparison by other groups using the same benchmark.

Automatic evaluation methods compare model-generated texts to pre-collected human-generated \emph{references} based on the same input data (e.g., images in image captioning) and use metrics based on n-gram overlap and semantic content matching.

N-gram overlap metrics measure the degree of matching between model-generated text and human-authored references. Take a few widely used metrics as examples. 
BLEU \citep{papineni2002bleu}, originally proposed for machine translation, is a weighted geometric mean of n-gram precision scores of a model-generated text with respect to the references. 
ROUGE \citep{lin2004rouge}, originally proposed for text summarization, focuses on recall rather than precision. It includes a large number of variants, including eight different n-gram counting methods to measure n-gram overlap between the generated text and reference. 
METEOR \citep{banerjee2005meteor} is originally proposed to address some of the issues of BLEU. It computes the harmonic mean of the unigram precision and recall, in which recall is weighted higher than precision. It has reported that METEOR yields higher correlation with human judgments.
CIDER \citep{vedantam2015cider}, originally proposed for image captioning, measures the similarity of a generated text against a set of references using a consensus-based protocol.

Semantic content matching metrics define the similarity between model-generated text and references by extracting explicit semantic information units from text beyond n-grams. An example widely used for image captioning and other VL tasks is SPICE \citep{anderson2016spice}. As illustrated in Figure~\ref{fig:chp2_spice}, instead of directly comparing the textual captions, SPICE parses model-generated captions and reference to form semantic scene graphs, encoding the objects, attributes, and relationships detected in image captions, then computes their matching score as the f-score over tuples in the candidate and reference scene graphs. SPICE has been shown to correlate well with human ratings.

\begin{figure*}[t!]
  \centering
    \includegraphics[width=0.6\linewidth]{figs/chp2_spice.jpg}
  \caption{Illustration of the SPICE metric used for evaluating image captioning results. Figure credit: \citet{anderson2016spice}.}
  \label{fig:chp2_spice}
\end{figure*}

\subsubsection*{Machine-Learned Metrics}

These metrics are based on machine-learned models, which are used digital judges to simulate human judges. This is an active research area although there is a hot debate whether machine learned models should be used at all for evaluation since these models can also be used for building the AI systems to be evaluated, thus leading to the problem of ``gaming the metrics''. As an example, Figure~\ref{fig:chp2_tiger} shows the image captioning evaluation result using various metrics, including a machine-learned metric, TiGEr~\citep{jiang2019tiger}. Instead of evaluating image captions based on n-gram overlap, TIGEr compares the candidate captions with references by mapping them into vectors in a common semantic space using a machine-learned text-image grounding model. As a result, TIGEr is able to detect the paraphrases based on the semantic meaning of caption sentences. 

\begin{figure*}[t!]
  \centering
    \includegraphics[width=0.8\linewidth]{figs/chp2_tiger.jpg}
  \caption{Illustration of the TIGER metric used for evaluating image captioning results. Two candidate captions are evaluated. Candidate (a) correctly describes image content, but contains many words that are not in the references. Candidate (b) substantially overlaps the references, but contains hallucinations (``a woman with straight hair''). Figure credit: \citet{jiang2019tiger}.}
  \label{fig:chp2_tiger}
\end{figure*}

\subsection{Evaluation of Image Generation}

Consider a text-to-image generation model $f(\theta)$, which produces image $y$ based on text caption $x$ as $y = f(x; \theta)$. 
Similar to the evaluation of text generation, the quality of  generated images is measured via  
\begin{itemize}
    \item \textbf{intrinsic evaluation:} how visually realistic these images are, and
    \item \textbf{extrinsic evaluation:} how good the image illustrate the text caption, or how semantically relevant the generated image is with respect to its conditioned caption.
\end{itemize}

Inception Score (IS) \citep{salimans2016improved} and Fréchet Inception Distance (FID)~\citep{heusel2017gans} are among the two most commonly used metrics for intrinsic evaluation while R-precision is widely used for extrinsic evaluation.

IS involves using a pre-trained image classification model (e.g., the Inception V3 model in \citet{salimans2016improved}) to classify the generated images. 
Given a collection of generated images $y \in \mathcal{Y}$, the model computes for each image-class pair a conditional probability of image $y$ belonging to $c$, $P(c|y)$, to capture two properties:
\begin{itemize}
    \item Quality: how much does an image look like a specific object class? 
    \item Diversity: does the collection $\mathcal{Y}$ cover a wide range of objects?
\end{itemize}

Images that are more easily classified as one class over all the other classes are considered higher quality. As such, the conditional probability of all generated images in the collection should have  a conditional label distribution $P(c|y)$ with low entropy.
On the other hand, we expect the model to generate diverse images. So the marginal probability (i.e., the probability distribution of all images in $\mathcal{Y}$) ${\int P(c|y = f(x;\theta))\,dx}$.
The IS score is then computed as the KL-divergence between the two entropies. The IS score has a lowest value of $1.0$ and a highest value of the number of classes used by the classification model. For example, if the Inception v3 model supports the $1,000$ classes of the ILSVRC 2012 dataset, the highest inception score on that dataset is $1,000$.

One problem of IS is that it cannot detect intra-class mode collapse, i.e., a model that can generate only one image per class might still have a high IS score although it is desirable for many applications.

To address this problem, FID is proposed to improve IS by calculating the distance between the feature vectors of real images and the feature vectors of generated images. Lower FID scores indicates higher quality of generated images as they are more similar to the real ones. The feature vectors can be extracted from images using pre-trained models, such as the Inception V3 model or most of the VL models described in this book.

Since neither IS nor FID can measure the semantic relevance between a generated image and its conditioned text description, R-precision has been widely used as a complementary metric for evaluating text-to-image models \citep[e.g.,][]{xu2018attngan,zhang2017stackgan}.

R-precision is a common evaluation metric for ranking retrieval results. For a given query topic Q, R-precision is the precision at $R$, where $R$ is the number of relevant documents for Q. If there are $r$ relevant documents among the top-$R$ retrieved documents, then R-precision is $r/R$.
To evaluate a text-to-image generation model, we use a generated image to query relevant text captions (e.g., the text caption conditioned on which the image is generated) among a collection of texts using a pre-trained VL model, and calculate the R-precision. 

% \subsection{Evaluating Generated Videos}

\section{Vision-Language Processing Basics}
\label{chp2-sec:basics}

We describe language and vision processing techniques that serve as the building blocks of the VL models and VLP methods described in the later chapters, including text feature extraction, vision feature extraction, and text and vision feature fusion. 

\subsection{Text Feature Extraction}

Text feature extraction is performed using a text encoder. Most popular text encoders use pre-trained language models. For example, the BERT-based encoder~\citep{devlin2018bert} encodes text in three step. 
\begin{enumerate}[leftmargin=*]
    \item An input text string is segmented into a sequence of sub-word tokens using byte pair encoding (BPE) and a \texttt{[CLS]} token is inserted at the beginning of the sequence. 
    \item The token sequence is converted to a sequence of continuous embedding vectors using BERT's embedding layer. 
    \item The embedding vectors are then fed into a stack of Transformer layers to produce contextual feature vectors, one for each token. The feature vector of \texttt{[CLS]} is often used as the representation of the entire text string.
\end{enumerate}

Depending on how we view text strings are structure, different neural models can be used for text encoding~\cite{minaee2021deep}. Just name a few below. 

\begin{itemize}[leftmargin=*]
    \item Feed-forward networks view a text string as a bag of words. Thus, they take the sum or average of token vectors as the representation of the text string.
    \item RNN-based models view text as a sequence of words, and are intended to capture word dependencies and text structures. 
	\item CNN-based models are trained to recognize patterns in text, such as key phrases.
	\item Graph neural networks (GNNs) are designed to capture internal graph structures of natural language, such as syntactic and semantic parse trees.
\end{itemize}

\subsection{Image Feature Extraction}

Image feature extraction is performed by an image encoder. Similar to text encoding, depending on how we view an image being structured, different types of image features can be extracted.

\begin{itemize}[leftmargin=*]
    \item Region features are extracted using pre-trained object detectors (e.g., Fast R-CNN \citep{girshick2015fast}) if we are interested in encoding the objects and their relations presented in the image.
    \item Grid features can be extracted from pre-set image grids using pre-trained CNNs (e.g., ResNet~\citep{he2016deep}) if we view an image as uniformly-arranged pixel arrays.
    \item Patch features are extracted from evenly split image patches via Vision Transformer (ViT) and its variants \citep{dosovitskiy2020image}. Patch features differ from grid features mainly in how they are extracted. While grid features are extracted from CNN-generated feature maps, patch features are extracted via contextual embedding of visual tokens (image patches) using multi-layer Transformer models.
    \item \citet{li2019relation} models an image as a graph using GNNs for VL reasoning tasks.
\end{itemize}

\subsection{Video Feature Extraction}

A video clip consists of a sequence of frames (images). Thus, we can extract for each frame 2D or 3D visual features such as region features or patch features as described above. Then the video is represented using the concatenation of the visual features of its frames.

%Two commonly used features are 
%\begin{itemize}[leftmargin=*]
%    \item 2D/3D grid features using CNNs/ResNet, and
%	\item Patch features using ViT.
%\end{itemize}

\subsection{Vision-Language Feature fusion}

Feature fusion aims at modeling inter-modality context. The methods can be grouped into three categories.

\begin{itemize}[leftmargin=*]
    \item Simple fusion uses simple concatenation and element-wise product for feature fusion. 
	\item Bilinear pooling \citep{fukui2016multimodal} allows all elements of text and vision vectors to interact with each other in a multiplicative way via outer product. However, the high dimensional representation (e.g., due to long text and/or high-resolution images) leads to an infeasible number of parameters to learn. Thus, various methods are proposed to reduce the computation cost by e.g., projecting the outer product to a lower dimensional space and avoid computing the outer product directly.
	\item Cross-modal attention \citep[e.g.,][]{yang2016stacked,lu2016hierarchical,nguyen2018improved,anderson2018bottom} is the most popular fusion method. Compared to simple fusion, attention models construct a more informative VL-joint representation since higher weights are put on the visual regions that are more useful to solve the task. For example, in VQA the vision regions that are more relevant to input question have higher weights. 
\end{itemize}

\section{Task-Specific VL Models}
\label{chp2-sec:task-specific-models}

We use VQA and image captioning as examples to review task-specific VL models that had been developed before the large-scale pretrained language models or VLP methods are widely used for VL tasks.
Early task-specific VL models differ in text features they used, vision features used, and how vision and text features are fused.

\subsection{VQA}

Given an image-question pair, VQA requires answering a question based on the image. Most studies treat VQA as a classification problem on a predefined answer set. For example, VQA v2 \citep{goyal2017making} has around 2K predefined answers.
A typical architecture of VQA systems is shown in Figure~\ref{fig:chp2_vqa}.

The fundamental research challenge of VQA is to obtain a joint representation of image and language (the question). Researchers in this field pursued various ways to encode and fuse image and language, which have laid the foundation for the following VLP models, as described in the rest of this paper. Most works in this field encode image and language independently and then fuse them. 

%\begin{itemize}[leftmargin=*]
%    \item Early models using global image representation and simple fusion \citep{antol2015vqa,malinowski2015ask},
%    \item The models based on bilinear pooling, such as the winner of 2016 VQA challenge \citep{fukui2016multimodal}, and
%    \item The attention-based methods, such as the stacked attention networks \citep{yang2016stacked}.
%\end{itemize}

Early VQA models \citep[e.g.,][]{antol2015vqa,malinowski2015ask,ren2015exploring} use global image representation and simple feature fusion methods including element-wise product or sum, and concatenation of image and text features. 
As illustrated in Figure~\ref{fig:chp2_vqa1}., the model uses a CNN (VGGNet) to encode input images and an RNN/LSTM model to encode questions. Both the question and image features are transformed to a common space and fused via element-wise multiplication. The fused features are fed to the classifier, which consists of a fully connected layer followed by a softmax layer, to predict the answer.

\begin{figure*}[t!]
  \centering
    \includegraphics[width=0.8\linewidth]{figs/chp2_vqa1.jpg}
  \caption{An example of the VQA models that use global image representation and simple feature fusion. Figure credit: \citet{antol2015vqa}.}
  \label{fig:chp2_vqa1}
\end{figure*}

\citet{fukui2016multimodal} argue that these simple feature fusion methods are not expressive enough to fully capture the complex associations between images and texts. Thus, they propose to use bilinear pooling to obtain a joint representation by computing the outer product between image and text feature vectors. For efficiency, bilinear pooling is approximated by randomly projecting image and text vectors to a higher dimensional space and then convolving them efficiently by using element-wise product in the Fast Fourier Transform space. The method, termed as Multimodal Compact Bilinear (MCB) pooling, is illustrated in Figure~\ref{fig:chp2_vqa2}. MCB is the winner of 2016 VQA challenge, and helps popularize the use of bilinear pooling for VL feature fusion.

\begin{figure*}[t!]
  \centering
    \includegraphics[width=0.6\linewidth]{figs/chp2_vqa2.jpg}
  \caption{Illustration of the Multimodal Compact Bilinear (MCB) pooling model for VQA, which use an approximated bilinear pooling method for image and text feature fusion. Figure credit: \citet{fukui2016multimodal}.}
  \label{fig:chp2_vqa2}
\end{figure*}

\citet{yang2016stacked} propose the first attention-based model for VQA. The model is motivated by the observation that an image usually contain multiple regions that represent particular objects or concepts, and the answer to a question is often related only to one or a few regions. As illustrated in Figure~\ref{fig:chp2_vqa3}, the image contains objects like \texttt{bicycle}, \texttt{window}, \texttt{street}, \texttt{baskets} and \texttt{dogs}. To answer the question \texttt{what are sitting in the basket on a bicycle}, the model only needs to pay attention to the regions related to \text{basket}, \text{bicycle} and the concept of \texttt{sitting in}. Thus, \citet{yang2016stacked} have developed a Stacked Attention Network (SAN) which consists of multiple question-guided layers each of which can attend to the image regions useful to answer the question. SAN helps popularize the use of attention models and use of region or object features for VQA \citep[e.g.,][]{anderson2018bottom,lu2016hierarchical,shih2016look}.   

\begin{figure*}[t!]
  \centering
    \includegraphics[width=0.6\linewidth]{figs/chp2_vqa3.jpg}
  \caption{Illustrate of Stack Attention Network (SAN), the first attention-based model for VQA. Figure credit: \citet{yang2016stacked}.}
  \label{fig:chp2_vqa3}
\end{figure*}


\subsection{Image Captioning}

The task is to generate a caption for an image. A caption is a text string that describes the content of the image including objects of interest, their behaviors, and the relations among them.

%\begin{itemize}[leftmargin=*]
%    \item Early modular systems, e.g., \citep{fang2015captions}.
%    \item The encoder-decoder models inspired by neural machine translation. E.g., \cite{xu2015show} propose the first method leveraging attention over gird features. But, global CNN feature has an obvious weakness because the decoder cannot focus on important regions of an image as humans do.
%    \item The bottom-up and top-down attention model \citep{anderson2018bottom}. Splitting an image into equally-sized grids is a naive way to perform attention because grids align poorly with objects. To address this problem, some researchers seek to align attention with more meaningful regions. \cite{anderson2018bottom} proposed a bottom-up and top-down attention (BUTD) approach to aligning attention with salient regions that are acquired with a detection model. BUTD extracts region features with a Faster-RCNN \citep{ren2015faster} model pre-trained on Visual Genome \citep{krishna2017visual}. Because detected object regions normally contain meaningful visual concepts and align better with human language, BUTD significantly improves the performance of both image captioning and VQA. Therefore, the pre-trained detector is widely adopted by subsequent VL studies. 
%\end{itemize}

Most of the early image captioning systems use a modular architecture \citep[e.g.,][]{farhadi2010every,kulkarni2013babytalk,fang2015captions} which typically consists of modules developed separately for detecting objects or concepts in images and generating captions using rules or machine learned models, respectively. As illustrated in Figure~\ref{fig:chp2_ic1}, the Microsoft system \citep{fang2015captions} generates image captions in three steps. First, a machine-learned word detector generates from an input image a set of words commonly found in image captions. Second, a maximum-entropy language model is used to form sentences (candidate captions) using the detected words. Third, a vision-language deep structured semantic model (DSSM) \citep{huang2013learning} trained on image-caption pairs is used to rank the candidate captions based on semantic similarities between the candidate captions and the image.

\begin{figure*}[t!]
  \centering
    \includegraphics[width=0.6\linewidth]{figs/chp2_ic1.jpg}
  \caption{Illustration of Microsoft's modular image captioning system. Figure credit: \citet{fang2015captions}.}
  \label{fig:chp2_ic1}
\end{figure*}

The first set of deep learning models for image captioning \citep[e.g.,][]{vinyals2015show,xu2015show} is inspired by the encoder-decoder models, also known as \emph{Seq2Seq}, which are originally developed for machine translation \citep{sutskever2014sequence,bahdanau2014neural}. As illustrated in Figure~\ref{fig:chp2_ic2}, the model uses an CNN-based encoder (e.g., GoogleNet \citep{szegedy2015going}) to extract grid features from an input image, and a RNN-based decoder to generate a caption based on the image features. Similar to the use of attention models in VQA, the encoder-decoder image captioning models are enhanced by incorporating an attention mechanism in the decoder so that the caption can be generated based on the image regions of objects and concepts of interest. Compared to those early modular systems, encoder-decoder models are advantageous in that they can be trained end-to-end on image captioning pairs.

\begin{figure*}[t!]
  \centering
    \includegraphics[width=0.7\linewidth]{figs/chp2_ic2.jpg}
  \caption{Illustration of the attention-enhanced encoder-decoder model for image captioning. Figure credit: \citet{xu2015show}.}
  \label{fig:chp2_ic2}
\end{figure*}

The model of \citet{anderson2018bottom} is among the first that uses region features extracted by a pre-trained object detector for image captioning. It takes a bottom-up and top-down (BUTD) attention approach to aligning attention with salient regions, which are extracted using a pre-trained Faster-RCNN \citep{ren2015faster} model. Compared to the pre-set grids used by early neural image captioning models using grid or patch image features, the detected object regions often contain more meaningful visual concepts and align better with human language, as illustrated in Figure~\ref{fig:chp2_ic3}. As a result, BUTD significantly improves the performance of image captioning. Therefore, the pre-trained detector is widely adopted by other VL studies afterwards.

\begin{figure*}[t!]
  \centering
    \includegraphics[width=0.7\linewidth]{figs/chp2_ic3.jpg}
  \caption{Example of the detected regions used in the BUTD model. Each bounding box is labeled with an attribute class followed by an object class. Only the feature vectors, not the predicted labels, are used for image captioning. Figure credit: \citet{anderson2018bottom}.}
  \label{fig:chp2_ic3}
\end{figure*}

%\section{Summary}

%[Jianfeng: need to add main references. e.g., for image captioning, we can case study MSR's modular, bottom-up systems and Google's encoder-decoder (show and tell) system. We can also describe early VQA systems that top the leaderboard (before 2018, e.g., MSR's up-down model -- tips and tricks from VQA in 2017, FB's A-star system (Pythia) in 2018). Take Image Captioning and VQA as examples. ]

